Line Search for Averaged Operator Iteration

Many popular first order algorithms for convex optimization, such as forward-backward splitting, Douglas-Rachford splitting, and the alternating direction method of multipliers (ADMM), can be formulated as averaged iteration of a nonexpansive mapping. In this paper we propose a line search for averaged iteration that preserves the theoretical convergence guarantee, while often accelerating practical convergence. We discuss several general cases in which the additional computational cost of the line search is modest compared to the savings obtained.

==> line_search.tex <==
%% PAPER VERSION

%\xdef\optresnorm{1000}
%\xdef\optt{1}
\xdef\one{1}

%\pgfmathparse{1+(4-1)*6.25}
%\edef\opttex{\pgfmathresult}
%\node[right] at ({\radius*0.84},{\radius*(0.02-0.02*(\maxlssteps+1))}) {\opttex};
\foreach \t in {1,2,...,\maxlssteps} {


% POINT x_k+1*res_k IN ppx_k

\pgfmathparse{\ppxone+(\t-1)*\resone*6.25}
%\pgfmathparse{\xone+\t*\resone}
\edef\xlsone{\pgfmathresult}
\pgfmathparse{\ppxtwo+(\t-1)*\restwo*6.25}
%\pgfmathparse{\xtwo+\t*\restwo}
\edef\xlstwo{\pgfmathresult}

%\node at (0.7,0.05) {\xlstwo};
%\node at (0.85,0.05) {\xlstwo};

% mark starting point
\marker{(\xlsone,\xlstwo)}{0.01};
%\node[left] at (\xlsone,\xlstwo) {$\hat{x}_{\t}^{\i}$};

% PROJECT ON LINE
\edef\pxlsone{\xline};
\pgfmathparse{1*\xlstwo}
\edef\pxlstwo{\pgfmathresult}
% END PROJECT ON LINE
% mark projection on line
\marker{(\pxlsone,\pxlstwo)}{0.01};
%\node[right] at (\pxlsone,\pxlstwo) {$\Pi_Cx_{\t}^{\i}$};

% PROJECT ON CIRCLE
\pgfmathparse{sqrt(\pxlsone*\pxlsone+\pxlstwo*\pxlstwo)};
\edef\pxlsnorm{\pgfmathresult};
\pgfmathparse{\pxlsone*\radius/\pxlsnorm};
\xdef\ppxlsone{\pgfmathresult};
\pgfmathparse{\pxlstwo*\radius/\pxlsnorm};
\xdef\ppxlstwo{\pgfmathresult};
% END PROJECT ON CIRCLE
% mark projection on circle
\marker{(\ppxlsone,\ppxlstwo)}{0.01};
%\node[above left] at (\ppxlsone,\ppxlstwo) {$x_{\t}^{2}$};

\pgfmathparse{\one}
\ifx\t\pgfmathresult
\else
\node[left] at (\ppxlsone,\ppxlstwo) {$x_{\t}^1$};
\fi

% DRAW STEPS
\draw[-latex] (\xlsone,\xlstwo)--(\pxlsone,\pxlstwo);
\draw[-latex] (\pxlsone,\pxlstwo)--(\ppxlsone,\ppxlstwo);
\draw[-latex] (\xlsone,\xlstwo)--(\ppxlsone,\ppxlstwo);

% compute residual
\pgfmathparse{\ppxlsone-\xlsone};
\edef\reslsone{\pgfmathresult};
\pgfmathparse{\ppxlstwo-\xlstwo};
\edef\reslstwo{\pgfmathresult};
\pgfmathparse{sqrt(\reslsone*\reslsone+\reslstwo*\reslstwo)};
\xdef\reslsnorm{\pgfmathresult};
% output residual
\node[right] at ({\radius*0.84},{\radius*(0.02-0.02*\t)}) {$\|r_{\t}^{1}\|=\reslsnorm$};





%\node[right] at ({\radius*0.6},{\radius*(-0.15)}) {$\|r_{\rm{opt}}^{1}\|=\optre%snorm$};
%\pgfmathparse{1+(\optt-1)*\i*(sqrt(\i))*0.3}
%\edef\trueoptt{\pgfmathresult}
%\node[right] at ({\radius*0.6},{\radius*(-0.2)}) {$t_{\rm{opt}}=\trueoptt$};



}
